Concentration of Measure Techniques and Applications

Concentration of measure is a phenomenon in which a random variable that depends in a smooth way on a large number of independent random variables is essentially constant. The random variable will "concentrate" around its median or expectation. In this work, we explore several theories and applications of concentration of measure. The results of the thesis are divided into three main parts. In the first part, we explore concentration of measure for several random operator compressions and for the length of the longest increasing subsequence of a random walk evolving under the asymmetric exclusion process, by generalizing an approach of Chatterjee and Ledoux. In the second part, we consider the mixed matrix moments of the complex Ginibre ensemble and relate them to the expected overlap functions of the eigenvectors as introduced by Chalker and Mehlig. In the third part, we develop a $q$-Stirling's formula and discuss a method for simulating a random permutation distributed according to the Mallows measure. We then apply the $q$-Stirling's formula to obtain asymptotics for a four square decomposition of points distributed in a square according to the Mallows measure. All of the results in the third part are preliminary steps toward bounding the fluctuations of the length of the longest increasing subsequence of a Mallows permutation.

==> urcsmacros.tex <==
%
% urcsmacros
%
% author: Lawrence A. Crowl
% last updated: 28 April 1990
%
% BibTeX
%
\newcommand{\BibTeX}{{B\kern-.0833em{\sc ib}\kern-.1667em%
T\kern-.1667em\lower.5ex\hbox{E}\kern-.125emX}}
%
% SLiTeX
%
\newcommand{\SliTeX}{{\rm S\kern-.06em{\sc l\kern-.035emi}\kern-.06em
T\kern -.1667em\lower.7ex\hbox{E}\kern-.125emX}}
%
% UNIX
%
\newcommand{\UNIX}{{\sc Unix}}
%
% trademark
%
\newcommand{\trademark}{$^{\rm TM}$}
%
% singlespacing (for use in doublespaced documents)
%
\def\doublespacefactor#1#2{%
\newenvironment{singlespace}{\baselineskip #2\baselineskip}%
{\par \baselineskip #1\baselineskip}%
\par \baselineskip #1\baselineskip}
%
% various latin abbreviations
%
\def\adhoc{{\em ad hoc}}
\def\aposteriori{{\em a posteriori}}
\def\apriori{{\em a priori}}
\def\Cf{{\em Cf.}}
\def\cf{{\em cf.}}
\def\Eg{{\em E.g.}}
\def\eg{{\em e.g.}}
\def\etal{{\em et al.}}
\def\etc{{\em etc.}}
\def\Ibid{{\em Ibid.}}
\def\ibid{{\em ibid.}}
\def\Id{{\em Id.}}
\def\id{{\em id.}}
\def\Ie{{\em I.e.}}
\def\ie{{\em i.e.}}
\def\Loccit{{\em Loc.\ cit.}}
\def\loccit{{\em loc.\ cit.}}
\def\Opcit{{\em Op.\ cit.}}
\def\opcit{{\em op.\ cit.}}
\def\qv{{\em q.v.}}
\def\Qv{{\em Q.v.}}
\def\viz{{\em viz.}}
%
% andbreak  (for breaking author lists)
%
\def\andbreak{%% \begin{tabular}
\end{tabular}\\\begin{tabular}[t]{c}%% \end{tabular}
}
%
% titlequote
%
\def\titlequote#1{\hfill
\parbox{4in}{\begin{flushright}{\small\it #1}\end{flushright}}}
%
% weekdaystring
%
% Dump the day of the week in string form.
% This macro is only valid from 1901 A.D. through 2099 A.D.
%
\def\weekdaystring#1#2#3{{% extra brace saves enclosing register state
%
% days through the end of the year
% days := current year * 365
\count10=#3%
\multiply\count10 by 365%
% leap years := year / 4
\count11=#3%
\divide\count11 by 4%
% days := days + leap years
\advance\count10 by \count11
%
% find out if the current year is a leap year
% last leap year := leap years * 4
\count12=\count11%
\multiply\count12 by 4
% years since last leap year := current year - last leap year
\count13=#3%
\advance\count13 by -\count12%
% years since last leap year equals zero when current year is a leap year
%
% subtract off those days in this month and the following months
% days = days - following days [ is leap ] [ current month ]
\ifcase#2%
\or\ifcase\count13\advance\count10 by -366% leap January
\else\advance\count10 by -365% normal January
\fi%
\or\ifcase\count13\advance\count10 by -335% leap February
\else\advance\count10 by -334% normal February
\fi%
\or\advance\count10 by -306% March
\or\advance\count10 by -275% April
\or\advance\count10 by -245% May
\or\advance\count10 by -214% June
\or\advance\count10 by -184% July
\or\advance\count10 by -153% August
\or\advance\count10 by -122% September
\or\advance\count10 by -92% October
\or\advance\count10 by -61% November
\or\advance\count10 by -31% December
\fi%
%
% update days by day of month
% days := days + current day
\advance\count10 by #1%
%
% find weekday number
% offset for initial day of the week
\advance\count10 by 5
% last monday := (current day / 7) * 7
\count14=\count10%
\divide\count14 by 7%
\multiply\count14 by 7
% weekday number := current day - last monday
\count15=\count10%
\advance\count15 by -\count14
%
% now dump out appropriate string
\ifcase\count15 Monday\or Tuesday\or Wednesday%
\or Thursday\or Friday\or Saturday\or Sunday\fi%
}}
%
% monthstring
%
% Dump the month in string form.
%
\def\monthstring#1{\ifcase#1\or January\or February\or March\or April\or May%
\or June\or July\or August\or September\or October\or November\or December\fi}
%
% dateWDMY
%
% Redefine \today as "weekdaystring daynumber monthstring yearnumber" format.
%
\def\dateWDMY{\def\today{\weekdaystring{\day}{\month}{\year}\space%
\number\day\space\monthstring{\month}\space\number\year}}
%
% dateDMY
%
% Redefine \today as "daynumber monthstring yearnumber" format.
%
\def\dateDMY{\def\today{\number\day\space\monthstring{\month}%
\space\number\year}}
%
% dateWMDY
%
% Redefine \today as "weekdaystring monthstring daynumber, yearnumber" format.
%
\def\dateWMDY{\def\today{\weekdaystring{\day}{\month}{\year}\space%
\monthstring{\month}\space\number\day,\space\number\year}}
%
% dateMDY
%
% Redefine \today as "monthstring daynumber, yearnumber" format.
%
\def\dateMDY{\def\today{\monthstring{\month}\space\number\day,%
\space\number\year}}
%
% dateMY
%
% Redefine \today as "monthstring yearnumber" format.
%
\def\dateMY{\def\today{\monthstring{\month}\space\number\year}}
%
% dateY
%
% Redefine \today as "yearnumber" format.
%
\def\dateY{\def\today{\number\year}}

